A Tensor-Train accelerated solver for integral equations in complex geometries

We present a framework using the Quantized Tensor Train (QTT) decomposition to accurately and efficiently solve volume and boundary integral equations in three dimensions. We describe how the QTT decomposition can be used as a hierarchical compression and inversion scheme for matrices arising from the discretization of integral equations. For a broad range of problems, computational and storage costs of the inversion scheme are extremely modest $O(\log N)$ and once the inverse is computed, it can be applied in $O(N \log N)$. We analyze the QTT ranks for hierarchically low rank matrices and discuss its relationship to commonly used hierarchical compression techniques such as FMM and HSS. We prove that the QTT ranks are bounded for translation-invariant systems and argue that this behavior extends to non-translation invariant volume and boundary integrals. For volume integrals, the QTT decomposition provides an efficient direct solver requiring significantly less memory compared to other fast direct solvers. We present results demonstrating the remarkable performance of the QTT-based solver when applied to both translation and non-translation invariant volume integrals in 3D. For boundary integral equations, we demonstrate that using a QTT decomposition to construct preconditioners for a Krylov subspace method leads to an efficient and robust solver with a small memory footprint. We test the QTT preconditioners in the iterative solution of an exterior elliptic boundary value problem (Laplace) formulated as a boundary integral equation in complex, multiply connected geometries.

==> CRZ14_TTIE_preamble.tex <==
\usepackage{pdf14}
\makeatletter
\newcommand\preserveCal[2]{
    \expandafter\newsavebox\csname box@\string#1\endcsname
    \expandafter\savebox\csname box@\string#1\endcsname{\ensuremath{\mathcal{#2}}}
    \expandafter\def\expandafter#1\expandafter
        {\expandafter\usebox\csname box@\string#1\endcsname}
}
\preserveCal{\Hmat}{H}

%%-- packages --------------------------------------------------------------------------------
\usepackage[T1]{fontenc}
\usepackage[bitstream-charter]{mathdesign} %\usepackage{charter} with no implication on math
\usepackage[scaled]{berasans}              %sans to complement bitstream-charter

\newlength{\alphabet}
\settowidth{\alphabet}{\normalfont abcdefghijklmnopqrstuvwxyz}
\geometry{textwidth=3.4\alphabet,top=1in, bottom=1.25in} %
%\geometry{top=1in, bottom=1.25in, left=1.25in, right=1.25in}
%\usepackage{fullpage}

\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amscd,mathrsfs} %,amssymb %conflict with charter fonts
\usepackage{mathtools}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it} %another typeface for calligraphic math with lowercase support.
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\usepackage{paralist}
\usepackage{siunitx}
\sisetup{table-format=4.2}
\sisetup{group-minimum-digits=3,group-separator={\,}}
\usepackage{xifthen}
\usepackage{float,ifdraft}
\usepackage[modulo]{lineno}
\usepackage[
  pdftitle={Tensor Train for Integral Equations},
  pdfcreator={pdflatex},
  pdfsubject={preprint},
  hyperindex = {true},
  colorlinks = {true},
  linkcolor = {blue},
  citecolor = {blue}
]{hyperref}

%%-- floats --------------------------------------------------------------------------------
\usepackage{graphicx}
\graphicspath{{./figs/}}
\usepackage{tabularx,booktabs,soul,multirow,collcell,dcolumn}
\usepackage[export]{adjustbox} %for proper alignment in figures/floats
\usepackage[scriptsize,tight]{subfigure}
\usepackage{caption}

\usepackage{pgf,tikz,pgfplots,import}
\pgfplotsset{compat=newest}
\pgfplotsset{plot coordinates/math parser=false}
\newlength\figureheight
\newlength\figurewidth
\usetikzlibrary{plotmarks}
\usetikzlibrary{pgfplots.groupplots}
\usetikzlibrary{matrix}
\usepgflibrary{fadings}
\usetikzlibrary{external}
%\tikzexternalize[prefix=figs/]

\usepgfmodule{oo}

%%disable hyperref in tikz figures
\makeatletter
\tikzset{
    every picture/.style={
        execute at begin picture={
            \let\ref\@refstar
        }
    }
}
\makeatother

\newcommand{\includepgf}[2][1]{
  \beginpgfgraphicnamed{#2}%
  \tikzsetnextfilename{tikz-external-#2}%
  \scalebox{#1}{\subimport{figs/}{#2.pgf}}%
  \endpgfgraphicnamed%
}

%% color for figures
%% \definecolor{plt-lc1}{rgb}{0.00000,0.44700,0.74100}%
%% \definecolor{plt-lc2}{rgb}{0.85000,0.32500,0.09800}%
%% \definecolor{plt-lc3}{rgb}{0.92900,0.69400,0.12500}%
%% \definecolor{plt-lc4}{rgb}{0.49400,0.18400,0.55600}%
%% better colors that work for bw
\definecolor{plt-lc1}{rgb}{0.0078,0.2980,0.7961}%blue
\definecolor{plt-lc2}{rgb}{1.0000,0.6431,0.2627}%orange
\definecolor{plt-lc3}{rgb}{1.0000,0.2863,0.5255}%purple
\definecolor{plt-lc4}{rgb}{0.6118,0.1765,1.0000}%violet

\usepackage{algorithm}
\usepackage{algorithmic}
% making the comments align
\newlength\commLen
\setlength\commLen{.6\linewidth} %can be adjusted locally
\newcommand{\algComment}[2][\commLen]{\hfill\parbox[t]{#1}{\raggedright\footnotesize\tt// #2}}
\renewcommand{\algorithmiccomment}[1]{\algComment{#1}}
\newcommand{\mcaption}[3]{
  \ifthenelse{\isempty{#2}}
             {\caption{\textit{#3}\label{#1}}}
             {\caption[#2]{\textit{{\sc #2.}~#3}\label{#1}}}
             }

\newcommand{\algcaption}[3]{
        \setcounter{ALC@unique}{0}
        \ifthenelse{\isempty{#3}}
                   {\caption[#1]{{\sc #2.} \label{#1}}}
                   {\caption[#1]{{\sc #2.} \newline\small{#3} \label{#1}}}
        }

%%-- referencing --------------------------------------------------------------------------------
%%%%% Hacking natbib b/c it's loaded by elsarticle but we want to use biblatex %%%%
%%%%% ignore natbib
\let\bibhang\relax
\let\citename\relax
\let\bibfont\relax
\let\Citeauthor\relax
\expandafter\let\csname ver@natbib.sty\endcsname\relax
\expandafter\let\csname c@author\endcsname\relax
%%%%% Loading biblatex
\usepackage[
  backend=bibtex,
  style=alphabetic,
  maxbibnames=99,
  maxcitenames=2,
  sorting=nyt,
  url=false,
  isbn=false,
  firstinits=true,
]{biblatex}
\renewcommand*{\multicitedelim}{\addcomma\space}
\renewcommand\citet[1]{\textcite{#1}}
\addbibresource{TTIE.bib}
\setlength\bibitemsep{2pt}
\renewcommand*{\bibfont}{\small}

\usepackage[capitalize]{cleveref}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Equation}{Equations}
\crefrangelabelformat{equation}{(#3#1#4--#5#2#6)}
\crefmultiformat{equation}{Eqs.~(#2#1#3)}{ and~(#2#1#3)}{, (#2#1#3)}{, and~(#2#1#3)}
\Crefmultiformat{equation}{Equations~(#2#1#3)}{ and~(#2#1#3)}{, (#2#1#3)}{, and~(#2#1#3)}
\crefname{review}{Response}{Responses} %the counter is review
\crefname{appendix}{}{} %els already has appendix in the name
\crefalias{ALC@unique}{line} %for algorithm line ref
\newcommand\pr[1]{\cref{#1}}
\renewcommand\Pr[1]{\Cref{#1}}

\def\figkeyword{Figure}
\newcommand\reftext[3][]{#3\hyperref[#2]{\ref{#2}#1}}

\def\bibsection{\section*{\refname}}

%% correct the target location so that it's above the line
%% from http://tex.stackexchange.com/questions/17057/hypertarget-seems-to-aim-a-line-too-low
\makeatletter
\newcommand{\hypertargetraised}[1]{\Hy@raisedlink{\hypertarget{#1}{}}}
\makeatother
%% macro to define and reference terms with document
\usepackage{relsize}
\newcommand\abbrev[2][\empty]{{#1\textsmaller{\uppercase{#2}}}}

%%-- annotation --------------------------------------------------------------------------------
\newcommand\authornote[2][Note]{\ifoptionfinal{}{\textcolor{cyan}{[{\bf #1:} #2]}}}
\newcommand\note[2][DRAFT]{\ifoptionfinal{}{\textcolor{orange}{[{\bf #1:} #2]}}}
\newcommand\ig[1]{\ifoptionfinal{}{\noindent\textcolor{gray}{//{\bf Ignore:}\\#1\\\noindent//}}}

\usepackage[color]{changebar}
\setlength{\changebarwidth}{4pt}
\definecolor{revcol1}{rgb}{0.0078,0.2980,0.7961}%blue
\definecolor{revcol2}{rgb}{0.6118,0.1765,1.0000}%violet
\definecolor{revcol3}{rgb}{1.0000,0.6431,0.2627}%orange

\def\revcolor{revcol1}
\newcommand\edit[2]{\textcolor{gray}{#1}\ \textcolor{\revcolor}{#2}}
\newcommand\editt[2]{\edit{\st{#1}}{#2}}
\newcommand\editm[2]{\textcolor{gray}{\ensuremath{#1}}\ \textcolor{\revcolor}{\ensuremath{#2}}}

%%-- environment --------------------------------------------------------------------------------
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\numberwithin{equation}{section}

%%-- macros --------------------------------------------------------------------------------
% Boxes for telescoping factorization diagram (D,L and R)
\newcommand{\lfr}[1]{\framebox[3em][c]{$#1$}}
\newcommand{\tfr}[1]{\fbox{\rule[-1em]{0pt}{2em}$#1$}}
\newcommand{\ltfr}[1]{\framebox[2\width][c]{\rule[-1em]{0pt}{2em}$#1$}}
% Bmatrices
\newcommand{\bbm}{\begin{bmatrix}}
\newcommand{\ebm}{\end{bmatrix}}
%
\newcommand\para[1]{\paragraph*{#1}}
\newcommand\lh[1]{\emph{#1}}
\newcommand\lbl[1]{\ensuremath{\mathrm{#1}}}
\newcommand\scie[2][1]{\ensuremath{#1e{#2}}}
\newcommand\sci[2][1]{\ensuremath{\ifthenelse{\equal{#1}{1}}{}{#1\times}10^{#2}}}
%
\DeclareMathOperator{\rank}{rank\,}
\DeclareMathOperator{\sinc}{sinc\,}
\DeclareMathOperator{\diric}{diric\,}
%
%Large and Huge math
\renewcommand\d{\ensuremath{\,d}}
\newcommand{\largemath}[1]{\text{\large $#1$}}
\newcommand{\hugemath}[1]{\text{\huge $#1$}}
\newcommand{\dimsym}[3]{{\scriptstyle #1}\stackrel{{\scriptstyle #2}}{#3}}
\newcommand\norm[2][{}]{\left\lVert #2 \right\rVert_{#1}}
\newcommand\card[1]{\left|#1\right|}
%
% math styles (for HSS and LR matrices)
\newcommand{\tA[1]}{\widetilde{#1}}
\newcommand{\hA[1]}{\hat{#1}}
\newcommand{\cA[1]}{\mathpzc{#1}}
\newcommand{\ttA[1]}{\mathtt{#1}}
\newcommand{\acc}{\varepsilon}
\def\defeq{\mathrel{\mathop :}=}
\newcommand\tensor[1]{\mathpzc{#1}}
\newcommand\set[1]{\mathscr{#1}}
\newcommand\tree[1]{\mathcal{#1}}
\newcommand\la[1]{\mathsf{#1}} %% Linear algebraic variable
\newcommand\laT[1]{\la{#1}}    %% Linear algebraic tensor
\newcommand\ordinal[1]{\ensuremath{#1\mathrm{th}}}
\def\bigO{\mathscr{O}}
\renewcommand\O[1]{\ensuremath{\bigO\left(#1\right)}}
\newcommand\0{\phantom{0}}
%
\def\vec{\ensuremath{\mathrm{vec}}}
\DeclareMathOperator{\reshape}{reshape\,}
\DeclareMathOperator{\diam}{diam\,}
\DeclareMathOperator{\diag}{diag\,}
\DeclareMathOperator{\dist}{dist\,}

\def\TTrain{tensor train}
\def\NTI{non-translation invariant}
\def\nystrom{Nystr\"om}
\def\Mdash/{\kern 0.05em---\kern 0.05em}
\def\matvec{matvec}
\def\Matvec{Matvec}
\def\tmatvec{\ensuremath{{T}_{mv}(N)}}
\newcommand\TT    {\abbrev{TT}}
\newcommand\QTT   {\abbrev{QTT}}
\newcommand\HIF   {\abbrev{HIF}}
\newcommand\HSS   {\abbrev{HSS}}
\newcommand\FMM   {\abbrev{FMM}}
\newcommand\FFT   {\abbrev{FFT}}
\newcommand\GMRES {\abbrev{GMRES}}
\newcommand\PDE   {\abbrev{PDE}}
\newcommand\twod  {\abbrev{2D}}
\newcommand\threed{\abbrev{3D}}

%\linenumbers
\setlength{\tabcolsep}{4pt}

%%------------------------------------------------------------------------------
%%- review and response tools
%%------------------------------------------------------------------------------
\usepackage{mdframed,framed}
\newcounter{review}[section]
\renewcommand{\thereview}{\thesection.\arabic{review}}

\newenvironment{review}
{\par\noindent\refstepcounter{review}\textbf{\thereview.}}
{\par\noindent\ignorespacesafterend}

\newenvironment{response}[1][\empty]{%
  \ifthenelse{\equal{#1}{\empty}}{\label{res:\thereview}}{\label{res:#1}}
  \begin{mdframed}[%
      frametitle={Response \thereview.},
      skipabove=\baselineskip plus 2pt minus 1pt,
      skipbelow=\baselineskip plus 2pt minus 1pt,
      linewidth=0.5pt,
      frametitlerule=true,
      frametitlebackgroundcolor=gray!30
    ]%
}{%
  \end{mdframed}
}

\newenvironment{revres}{%
\def\revcolor{revcol2}
\color{\revcolor}%
\ignorespaces%
}{\ignorespacesafterend}

